Compressed Latent Replays for Lightweight Continual Learning on Spiking Neural Networks

Rehearsal-based Continual Learning (CL) has been intensely investigated in Deep Neural Networks (DNNs). However, its application in Spiking Neural Networks (SNNs) has not been explored in depth. In this paper we introduce the first memory-efficient implementation of Latent Replay (LR)-based CL for SNNs, designed to seamlessly integrate with resource-constrained devices. LRs combine new samples with latent representations of previously learned data, to mitigate forgetting. Experiments on the Heidelberg SHD dataset with Sample and Class-Incremental tasks reach a Top-1 accuracy of 92.5% and 92%, respectively, without forgetting the previously learned information. Furthermore, we minimize the LRs' requirements by applying a time-domain compression, reducing by two orders of magnitude their memory requirement, with respect to a naive rehearsal setup, with a maximum accuracy drop of 4%. On a Multi-Class-Incremental task, our SNN learns 10 new classes from an initial set of 10, reaching a Top-1 accuracy of 78.4% on the full test set.

==> Tables/Acc_vs_past_samples.tex <==
        \begin{table}[t]
            \centering
            \caption{Memory-Accuracy tradeoff with variable $C_r$ and number of LRs in the Sample and Class-Incremental setup.}
            \begin{tabular}{|c|c|c|c|c|c|}

                \hline
                \textbf{$C_r$}   
                & \textbf{Past-samples}   
                & \textbf{5120}
                & \textbf{2560}
                & \textbf{1280}
                & \textbf{640}              \\

                \hline
                \multirow{2}{*}{\textbf{1:1}}
                & \textbf{Acc}   
                & XXX\%
                & XXX\%
                & XXX\%
                & XXX\%                   \\
                \cline{2-6}
                &\textbf{Mem}   
                & 1600 KB
                & 800 KB
                & 400 KB
                & 200 KB                      \\
                
                \hline
                \multirow{2}{*}{\textbf{1:5}}
                & \textbf{Acc}   
                & 88.88\%
                & 88.20\%
                & 87.64\%
                & 86.80\%                   \\
                \cline{2-6}
                &\textbf{Mem}   
                & 320 KB
                & 160 KB
                & 80 KB
                & 40 KB                      \\

                \hline
                \multirow{2}{*}{\textbf{1:10}}
                & \textbf{Acc}   
                & 87.60\%
                & 86.94\%
                & 86.42\%
                & 85.72\%                    \\
                \cline{2-6}
                &\textbf{Mem}   
                & 160 KB
                & 80 KB
                & 40 KB
                & 20 KB                      \\
                \hline


                \hline
                \textbf{$C_r$}   
                & \textbf{Past-samples}   
                & \textbf{5120}
                & \textbf{2560}
                & \textbf{1280}
                & \textbf{640}              \\

                \hline
                \multirow{2}{*}{\textbf{1:1}}
                & \textbf{Acc}   
                & XXX\%
                & XXX\%
                & XXX\%
                & XXX\%                   \\
                \cline{2-6}
                &\textbf{Mem}   
                & 1600 KB
                & 800 KB
                & 400 KB
                & 200 KB                      \\
                
                \hline
                \multirow{2}{*}{\textbf{1:5}}
                & \textbf{Acc}   
                & 88.88\%
                & 88.20\%
                & 87.64\%
                & 86.80\%                   \\
                \cline{2-6}
                &\textbf{Mem}   
                & 320 KB
                & 160 KB
                & 80 KB
                & 40 KB                      \\

                \hline
                \multirow{2}{*}{\textbf{1:10}}
                & \textbf{Acc}   
                & 87.60\%
                & 86.94\%
                & 86.42\%
                & 85.72\%                    \\
                \cline{2-6}
                &\textbf{Mem}   
                & 160 KB
                & 80 KB
                & 40 KB
                & 20 KB                      \\
                \hline
                
            \end{tabular}
            \label{tab:acc_mem_vs_past_samples}
        \end{table}

==> Tables/Tab_Class_Acc.tex <==
        \begin{table}[!ht]
            \centering
            \caption{Accuracy}
            \begin{tabular}{|c|c|c|c|c|c|c|}

                \hline
                \textbf{Class}   
                & \textbf{Past}
                & \textbf{New}
                & \textbf{Past}
                & \textbf{New}
                & \textbf{Past}
                & \textbf{New}              \\
                
                \hline
                \textbf{0}
                & 90.80\%
                & 0.00\%
                & 12.40\%
                & 100\%
                & 16.10\%
                & 100\%                   \\
                                
                \hline
                \textbf{1}
                & 90.40\%
                & 20.30\%
                & 85.20\%
                & 82.80\%
                & 76.30\%
                & 98.40\%                   \\

                \hline
                \textbf{2}
                & 84.60\%
                & 96.90\%
                & 20.40\%
                & 100\%
                & 8.10\%
                & 100\%                   \\
                
                \hline
                \textbf{3}
                & 86.00\%
                & 100\%
                & 85.20\%
                & 0.00\%
                & 84.80\%
                & 0.00\%                   \\

                \hline
                \textbf{4}
                & 90.00\%
                & 93.80\%
                & 25.20\%
                & 100\%
                & 16.10\%
                & 24.70\%                   \\

                \hline
                \textbf{5}
                & 90.20\%
                & 98.40\%
                & 84.40\%
                & 96.90\%
                & 82.90\%
                & 98.40\%                   \\

                \hline
                \textbf{6}
                & 90.20\%
                & 0.00\%
                & 28.40\%
                & 100\%
                & 23.60\%
                & 100\%                   \\

                \hline
                \textbf{7}
                & 83.10\%
                & 92.20\%
                & 91.20\%
                & 0.00\%
                & 90.60\%
                & 0.00\%                   \\

                \hline
                \textbf{8}
                & 89.00\%
                & 0.00\%
                & 30.50\%
                & 100\%
                & 27.90\%
                & 100\%                   \\

                \hline
                \textbf{9}
                & 88.20\%
                & 0.00\%
                & 88.10\%
                & 0.00\%
                & 88.40\%
                & 0.00\%                   \\

                \hline
                \textbf{10}
                & 91.80\%
                & 0.00\%
                & 22.60\%
                & 100\%
                & 15.00\%
                & 100\%                   \\

                \hline
                \textbf{11}
                & 89.70\%
                & 96.90\%
                & 92.60\%
                & 0.00\%
                & 91.20\%
                & 0.00\%                   \\

                \hline
                \textbf{12}
                & 85.10\%
                & 98.40\%
                & 50.00\%
                & 100\%
                & 52.20\%
                & 100\%                   \\

                \hline
                \textbf{13}
                & 87.70\%
                & 93.80\%
                & 83.60\%
                & 98.40\%
                & 83.00\%
                & 98.40\%                   \\

                \hline
                \textbf{14}
                & 88.00\%
                & 93.80\%
                & 16.80\%
                & 100\%
                & 14.40\%
                & 100\%                   \\

                \hline
                \textbf{15}
                & 88.20\%
                & 95.30\%
                & 89.20\%
                & 0.00\%
                & 88.00\%
                & 0.00\%                   \\

                \hline
                \textbf{16}
                & 91.10\%
                & 0.00\%
                & 33.20\%
                & 100\%
                & 31.60\%
                & 100\%                   \\

                \hline
                \textbf{17}
                & 91.40\%
                & 0.00\%
                & 88.40\%
                & 0.00\%
                & 89.00\%
                & 0.00\%                   \\

                \hline
                \textbf{18}
                & 88.30\%
                & 96.90\%
                & 24.50\%
                & 100\%
                & 17.20\%
                & 100\%                   \\

                \hline
                \textbf{19}
                & 87.50\%
                & 96.90\%
                & 87.70\%
                & 0.00\%
                & 87.90\%
                & 0.00\%                   \\
                
                \hline
                
            \end{tabular}
            \label{tab:acc_mem_vs_past_samples}
        \end{table}


        Reharsal training can provide a first solution to the problem of catastrophic forgetting. The technique consists of providing a sub-portion of the pre-training dataset every time the model is trained on a new sample. Figures  and  show the results obtained with different percentages of past examples. The interesting part is that this time, after an initial drop of around  15\% in the accuracy, the model learns again to recognize the examples seen during the pre-training phase, going back to its original value. At the same time it is able to learn the new samples, reaching almost the same accuracy of the other speakers.
    

    As expected, parametrizing the results with respect to the number of batches of past samples provided in input to the network during the incremental learning phase, the accuracy trend for the new speaker and for the ones seen during pre-training is opposite. So the higher the number of past batches provided the slower is the model to learn new samples, and the better it is able to remember the past ones. The trend is summarized in figure.


    As said before however, the main drawback of reharsal training is the large memory requirements: the batches of past samples need to be kept in memory to be used during the continual learning phase. To tackle the problem the core contribution of this paper is the application of latent replay, in particular the one presented by \textbf{Pellegrini et al.} to sSNN.
